Revisiting 3D Object Detection From an Egocentric Perspective

3D object detection is a key module for safety-critical robotics applications such as autonomous driving. For these applications, we care most about how the detections affect the ego-agent's behavior and safety (the egocentric perspective). Intuitively, we seek more accurate descriptions of object geometry when it's more likely to interfere with the ego-agent's motion trajectory. However, current detection metrics, based on box Intersection-over-Union (IoU), are object-centric and aren't designed to capture the spatio-temporal relationship between objects and the ego-agent. To address this issue, we propose a new egocentric measure to evaluate 3D object detection, namely Support Distance Error (SDE). Our analysis based on SDE reveals that the egocentric detection quality is bounded by the coarse geometry of the bounding boxes. Given the insight that SDE would benefit from more accurate geometry descriptions, we propose to represent objects as amodal contours, specifically amodal star-shaped polygons, and devise a simple model, StarPoly, to predict such contours. Our experiments on the large-scale Waymo Open Dataset show that SDE better reflects the impact of detection quality on the ego-agent's safety compared to IoU; and the estimated contours from StarPoly consistently improve the egocentric detection quality over recent 3D object detectors.

==> figures/analysis.tex <==
\begin{figure}[t]
    \centering
    \begin{tabular}{ccc}
            \begin{tabular}{c}
            \input{figures/sdeap_v_iouap} \\
            \footnotesize{(a) SDE-AP v.s IoU-AP} \\
            \input{tables/pp_v_pvrcnn} \\
            \footnotesize{(b) PP v.s PVRCNN}
            \end{tabular}
            &
            \begin{tabular}{c}
            \input{figures/fn_fp_of_all} \\
            \footnotesize{(c) FN/FP} \\
            \input{tables/tp_of_all} \\
            \footnotesize{(d) TP}
            \end{tabular}
            &
            \begin{tabular}{c}
            \input{figures/box_v_cvx} \\
            \footnotesize{(e) Box v.s Cvx}
            \end{tabular}
    \end{tabular}
    \caption{Analysis}
    \label{fig:Analysis}
\end{figure}

==> figures/box_v_cvx.tex <==
\includegraphics[width=0.27\textwidth]{images/box_v_cvx.png}
% \caption{SDE-AP v.s IoU-AP}
\label{fig:box_v_cvx}

==> figures/cvx_quali.tex <==
\begin{wrapfigure}{r}{0.3\textwidth}
    \centering
    \includegraphics[width=0.3\textwidth]{images/cvx_quali.png}
    \caption{Convex Visible Contour is prone to occlusion.}
    \label{fig:cvx_quali}
\end{wrapfigure}

==> figures/fn_fp_of_all.tex <==
\includegraphics[width=0.38\textwidth]{images/fn_fp_of_all.png}
\label{fig:fn_fp_of_all}

==> figures/sde_temporal.tex <==
\begin{wrapfigure}{r}{0.6\textwidth}
    \centering
    \includegraphics[width=0.45\textwidth]{images/sde_temporal.png}
    \caption{\textbf{Support distance errors at different time steps.} We see how visible contour's SDE significantly increases as the evaluation goes into the future frames , although its error at the T=0s is lower than the detector box.}
    \label{fig:sde_temporal}
\end{wrapfigure}

==> figures/sdeap_v_iouap.tex <==
\includegraphics[width=0.33\textwidth]{images/sdeap_v_iouap.png}
\label{fig:sdeap_v_iouap}

==> sections/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Sec.~\ref{sec:metrics} for practical trade-offs in using the expanded box as the ego-agent's shape and using aggregated points as ground truth to remove the need of human labeling. We also showed the limitation of the StarPoly model in Sec.~\ref{sec:starpoly_results} Results.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{We believe our work will benefit society by providing another perspective to evaluate detection and help set a higher safety standard for robotics and autonomous driving.}
    % setting a higher safety standard for the autonomous driving community.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

% \item If you are including theoretical results...
% \begin{enumerate}
%   \item Did you state the full set of assumptions of all theoretical results?
%     \answerTODO{}
% 	\item Did you include complete proofs of all theoretical results?
%     \answerTODO{}
% \end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{The code and the data are proprietary. We plan to release the code of computing the metrics upon acceptance.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Sec.\ref{sec:metrics}, Sec.\ref{sec:sde_analysis} and Sec.\ref{sec:egocentric_eval}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{Most of our experiments are deterministic. We report variance of the proposed StarPoly in the supplementary material. }
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{We include this information in the supplementary material for our proposed StarPoly model.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNA{We have followed the terms for using the Waymo Open Dataset for pure academic research purposes.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{We have followed the terms for using the Waymo Open Dataset for pure academic research purposes.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{We only use the Lidar point clouds and bounding box annotations which do not relate to personally identifiable information or offensive content.}
\end{enumerate}

% \item If you used crowdsourcing or conducted research with human subjects...
% \begin{enumerate}
%   \item Did you include the full text of instructions given to participants and screenshots, if applicable?
%     \answerTODO{}
%   \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
%     \answerTODO{}
%   \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
%     \answerTODO{}
% \end{enumerate}

\end{enumerate}

==> tables/pp_v_pvrcnn.tex <==
\resizebox{0.33\textwidth}{!}{%

\begin{tabular}{l|cc|cc}
\toprule
\multirow{2}{*}{Detector} & \multicolumn{2}{c|}{TP Acc.} & \multicolumn{2}{c}{FP/FN AP}  \\
                          & Near   & Far                 & Near   & Far                    \\ 
\midrule
PVRCNN                    & 0.9030 & 0.6753              & 0.9872 & 0.8762                 \\
PointPillar               & 0.9453 & 0.6781              & 0.9746 & 0.8002                 \\
\bottomrule
\end{tabular}

} %< resizebox
% \caption{PP v.s PVRCNN}
\label{tab:pp_v_pvrcnn}

==> tables/real_dataset.tex <==
\begin{table}
\begin{center}
\resizebox{0.45\textwidth}{!}{%

\begin{tabular}{l|cccc}
\toprule[1pt]
Method     & Precision $\uparrow$  & Recall $\uparrow$  & F-Score $\uparrow$  & Chamfer $\downarrow$   \\ 
\midrule
\midrule
Box        & 57.59                 & 100.00             & 69.98               & 0.00                   \\
ConvexHull & 95.41                 & 69.76              & 79.07               & 27.58                  \\
CvxNet     & -                     & -                  & -                   & -                      \\
OccNet2D   & 82.48                 & 95.11              & 86.91               & 2.34                   \\ 
\midrule
DOPS       & -                     & -                  & -                   & -                      \\
Comp.      & -                     & -                  & -                   & -                      \\ 
\midrule
SP         & 84.05                 & 97.78              & 88.85               & 1.00                   \\
NSP        & 84.62                 & 97.50              & 89.32               & 1.10                   \\
\bottomrule[1pt]
\end{tabular}

} %< resizebox
\end{center}
% \drawmyfilename{}
% \vspace{\baselineskip}
\caption{
Real Dataset Results.
}
\label{tbl:real_dataset}
\end{table}

==> tables/sde_box_v_cvx_old.tex <==

% \begin{wraptable}{r}{0.6\textwidth}

\begin{table}
\begin{center}
% \resizebox{0.5\textwidth}{!}{%

\begin{tabular}{l|cc|cc} 
\toprule
                            & \multicolumn{2}{c|}{\textbf{PV-RCNN}} & \multicolumn{2}{c}{\textbf{Ground Truth }}  \\
                            & Box   & CVC                           & Box   & CVC                                 \\ 
\midrule
mSDE of [$0m$, $10m$)       & 0.107 & 0.088                         & 0.068 & 0.077                               \\ 
\midrule
mSDE of [$10m$, $\infty m$) & 0.224 & 0.265                         & 0.142 & 0.213                               \\
\bottomrule
\end{tabular}

% } %< resizebox
\end{center}
% \drawmyfilename{}
% \vspace{\baselineskip}
\caption{
Quantitatively comparing mean support distance error (mSDE) between boxes and visible contours (cvx) at different ranges, from the egocentric perspective.
}
\label{tab:sde_box_v_cvx}
\end{table}

% \end{wraptable}

==> tables/synthetic_dataset.tex <==
\begin{table*}
\begin{center}
\resizebox{\textwidth}{!}{%

\begin{tabular}{l|cccc|cccc|cccc} 
\toprule[1pt]
\multirow{2}{*}{Method} & \multicolumn{4}{c|}{\textbf{Car} }                                                       & \multicolumn{4}{c|}{\textbf{Airplane} }                                                 & \multicolumn{4}{c}{\textbf{Watercraft} }                                                  \\
                        & Precision $\uparrow$  & Recall $\uparrow$  & F-Score $\uparrow$  & Chamfer $\downarrow$  & Precsion $\uparrow$  & Recall $\uparrow$  & F-Score $\uparrow$  & Chamfer $\downarrow$  & Precision $\uparrow$  & Recall $\uparrow$  & F-Score $\uparrow$  & Chamfer $\downarrow$   \\ 
\midrule
\midrule
Box                     & 49.00                 & 100.00             & 61.73               & 0.00                  & 9.67                 & 100.00             & 17.17               & 0.00                  & 60.42                 & 100.00             & 72.55               & 0.00                   \\
ConvexHull              & 95.56                 & 83.79              & 88.56               & 12.19                 & 45.94                & 83.47              & 56.59               & 11.67                 & 96.47                 & 76.66              & 84.21               & 13.36                  \\
CvxNet                  & -                     & -                  & -                   & -                     & -                    & -                  & -                   & -                     & -                     & -                  & -                   & -                      \\
OccNet2D                & 55.03                 & 94.53              & 66.63               & 2.54                  & 68.13                & 92.83              & 76.16               & 3.42                  & 69.09                 & 94.15              & 76.98               & 2.82                   \\ 
\midrule
DOPS                    & 92.30                 & 98.17              & 95.14               & 0.47                  & -                    & -                  & -                   & -                     & -                     & -                  & -                   & -                      \\
Comp.                   & -                     & -                  & -                   & -                     & -                    & -                  & -                   & -                     & -                     & -                  & -                   & -                      \\ 
\midrule
SP                      & 93.05                 & 98.92              & 95.48               & 0.50                  & 65.95                & 95.92              & 76.70               & 1.99                  & 73.69                 & 99.18              & 81.66               & 0.36                   \\
NSP                     & 89.45                 & 99.71              & 93.64               & 0.16                  & 68.68                & 95.85              & 78.70               & 1.96                  & 77.33                 & 98.76              & 84.51               & 0.58                   \\
\bottomrule[1pt]
\end{tabular}

} %< resizebox
\end{center}
% \drawmyfilename{}
% \vspace{\baselineskip}
\caption{
Synthetic Dataset Results. Precision, Recall, and F-Score are all reported in percentage ($\%$) at a threshold $\epsilon=1.2\text{e-}2$, where higher is better. Chamfer is the chamfer distance from the point cloud to the predicted shape, reported at $1\text{e-}3$ (\ie, $\times 1\text{e-}3$), where lower is better.
}
\label{tbl:synthetic_dataset}
\end{table*}

==> tables/tp_of_all.tex <==
\resizebox{0.38\textwidth}{!}{%

\begin{tabular}{l|cccccc} 
\toprule
       & PointPillar & PVRCNN & Signle-MVF & Multi-MVF & GT     & GT-Cvx  \\
\midrule
Near   & 0.9453      & 0.9030 & 0.9201     & 0.9562    & 0.9649 & 1.0000  \\
Global & 0.6781      & 0.6753 & 0.7031     & 0.7174    & 0.7626 & 0.8863  \\
\bottomrule
\end{tabular}

} %< resizebox
% \caption{PP v.s PVRCNN}
\label{tab:tp_of_all}
